Limits on anomalous trilinear gauge couplings from WW->e+e-, WW->emu, and WW->mu+mu- events from p-pbar collisions at sqrt(s)=1.96 TeV

Limits are set on anomalous WWgamma and WWZ trilinear gauge couplings using W+W- -> e+e-, W+W- -> e mu, and W+W- -> mu+mu- events. The data set was collected by the Run II D0 detector at the Fermilab Tevatron Collider and corresponds to approximately 250 inverse pb of integrated luminosity at sqrt(s) = 1.96 TeV. Under the assumption that the WWgamma couplings are equal to the WWZ couplings and using a form factor scale of Lambda = 2.0 TeV, the combined 95% C.L. one-dimensional coupling limits from all three channels are -0.32 < Delta kappa < 0.45 and -0.29 < lambda < 0.30.

==> list_of_visitor_addresses_r2.tex <==
% list_of_visitor_addresses_r2.tex                            7/19/06
%
\bibitem[*]{kurca}
On leave from IEP SAS Kosice, Slovakia.
\bibitem[\dag]{voutilainen}
Visitor from Helsinki Institute of Physics, Helsinki, Finland.
\bibitem[\ddag]{kozminski}
Visitor from Lewis University, Romeoville, IL, USA
%
\vskip 0.25cm

